Null-forms of conic systems in $\mathbb{R}^3$ are determined by their symmetries

We address the problem of characterisation of null-forms of conic $3$-dimensional systems, that is, control-affine systems whose field of admissible velocities forms a conic (without parameters) in the tangent space. Those systems have been previously identified as the simplest control systems under a conic nonholonomic constraint or as systems of zero curvature. In this work, we propose a direct characterisation of null-forms of conic systems among all control-affine systems by studying the Lie algebra of infinitesimal symmetries. Namely, we show that the Lie algebra of infinitesimal symmetries characterises uniquely null-forms of conic systems.

==> includes/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% ADDITIONAL PACKAGES %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsmath}

\usepackage[backend=bibtex,%
			style=alphabetic,%
			autolang=hyphen,%
			isbn=false,%
			date=year,%
			eprint=false,%
			]{biblatex}
			
\usepackage{hyperref} % need to be loaded after biblatex
\usepackage[nameinlink,capitalise,noabbrev]{cleveref}% must be after hyperef

\hypersetup{
    colorlinks,
    linkcolor={blue!80!black},
    citecolor={blue!80!black},
    urlcolor={blue!80!black},
    % filecolor=magenta,      
    % bookmarks=true,
    pdftitle={Null-forms of conic systems in R3 are determined by their symmetries},
    pdfauthor={Timothée Schmoderer, Witold Respondek},
    pdfsubject={We address the problem of characterisation of null-forms of conic 3-dimensional systems, that is, control-affine systems whose field of admissible velocities forms a conic (without parameters) in the tangent space. Those systems have been previously identified as the simplest control systems under a conic nonholonomic constraint or as systems of zero curvature. In this work, we propose a direct characterisation of null-forms of conic systems among all control-affine systems by studying the Lie algebra of infinitesimal symmetries. Namely, we show that the Lie algebra of infinitesimal symmetries characterises uniquely null-forms of conic systems.},
    pdfkeywords={Control-affine system, Conic systems, Feedback equivalence, Infinitesimal symmetries, Normal forms},
}

%\AtEveryBibitem{\clearfield{pages}}    % remove pages
\AtEveryBibitem{\clearfield{edition}}  % remove edition
\AtEveryBibitem{\clearfield{place}}    % remove place
\AtEveryBibitem{\clearfield{address}}  % remove address
\AtEveryBibitem{\clearfield{location}} % remove address 
\AtEveryCitekey{\clearlist{location}}
\AtEveryBibitem{\clearlist{location}}
\renewbibmacro{in:}{}				   % remove in
